Data-Driven Permissible Safe Control with Barrier Certificates

This paper introduces a method of identifying a maximal set of safe strategies from data for stochastic systems with unknown dynamics using barrier certificates. The first step is learning the dynamics of the system via Gaussian process (GP) regression and obtaining probabilistic errors for this estimate. Then, we develop an algorithm for constructing piecewise stochastic barrier functions to find a maximal permissible strategy set using the learned GP model, which is based on sequentially pruning the worst controls until a maximal set is identified. The permissible strategies are guaranteed to maintain probabilistic safety for the true system. This is especially important for learning-enabled systems, because a rich strategy space enables additional data collection and complex behaviors while remaining safe. Case studies on linear and nonlinear systems demonstrate that increasing the size of the dataset for learning the system grows the permissible strategy set.

==> bin/activeLearning.tex <==
\begin{problem}[Safe Active Learning]
\label{prob:2}
Given a set of data $D,$ probability threshold $p^*,$ and time horizon $N\in \mathbb{N}$, find a strategy $\pi$ such that:
\begin{align*}
    \label{eq:active learning}
    \pi \in \arg \min_{\pi} \max_{x\in  \ProbControlSafeSet{\pi}} \sigma^2_D(x,\pi(x)).
\end{align*}
\begin{align*}
    % \label{eq:active learning}
   \forall {x\in  \ProbControlSafeSet{\pi}},  \pi \in \arg \min_{\pi}  \sigma^2_D(x,\pi(x)).
\end{align*}
\end{problem}

Collection of data in states where the posterior variance is high is a widely-used exploration criterion in experimental design and shown to lead to optimality guarantees in terms of number of sample required for exploration \cite{srinivas2012information}. 
Problem \ref{prob:2} constrains this criterion to only those states and control actions that lead to safe behavior according to the current information.
% That is, constraint $x \in \ProbControlSafeSet{\pi}$ in \eqref{eq:active learning} requires that the choice of control strategy $\pi$ at current state $x$ is limited to those that keep the system in the N-invariant set.
Hence, solving Problem~\ref{prob:2} iteratively allows for efficient exploration to reduce uncertainty with (probabilistic) safety guarantees.
Then, as new data are collected, the strategy and probabilistic N-invariant set are updated according to the new posterior distribution of System~\eqref{eq:system}.

\ml{Note that updates to the strategy and invariant set can be done in every $N$ steps instead of every step, reducing the burden of `online' computation, also making the updates more impactful since N additional data is available rather than 1 data point.}\LL{Issue with having that inside Problem 2 is that it becomes not easy to be formal and have a criteria to optimize. But we can discuss whenever you are free. }

\begin{remark}
We stress that a possible option would have been to consider a longer time horizon, and only states from which trajectories will stay safe with high probability. However, especially when no many data are available, this approach may become overly conservative compared to that considered in Problem 2. 
\LL{Improve and expand this discussion}
\ml{we could make multiple points in this remark. Let's discuss it.}.
\end{remark}

%\LL{As we consider $N$ time steps need to think at why we simply do not simply use the set of states from which the system will remain in the safe set. What is the advantage of considering  $\ProbControlSafeSet{\pi}$ instead of this? }
%\ml{We could extend the def. to $N \in \mathbb{N} \cup \{\infty\}$, and we could say, in practice, due to large uncertainty (finite amount of data), the $\infty$-invariant set is usually empty.}

%\ml{next, we can define Problem 2 to find the set of all control strategies as well as the N-invariant set for a given $D$, $N$, and $p^*$.}

%\ml{Problem 3: actively collect data to expand N-variant set... need to think about a formal way of stating it.}





\LL{From here it is the old version}


The first problem is identifying the safety-invariant set in a data-driven manner.

\begin{problem}[Safety-Invariant Set]
% \label{prob:2}
Let $f$ satisfy Assumption~\ref{ass:f}. Given the dataset $\dataset$, horizon $N$, and threshold $p^*$, find the probabilistic safety-invariant set $\ProbControlSafeSet{\pi}$ for Process~\eqref{eq:system}.
\end{problem}

The safety-invariant set $\ProbControlSafeSet{\pi}$ provides initial conditions from which Process~\eqref{eq:system} can be deployed with safety invariance guarantees. 
Since the given dataset $\dataset$ may be small or have limited coverage of the state-control hyperspace, our next problem focuses on collecting additional data to grow $\ProbControlSafeSet{\pi}$.
This is realized by choosing control inputs that have the most potential to reduce the uncertainty of $f$.
The second problem is to collect the most informative data from an initial state in the safety-invariant set. 

\JS{I've checked several papers on active learning with GPs, and none are specific on the AL problem beyond ``we want to get the best info''. I've updated the text to make it clear we want to stay in the invariant set.}

\begin{problem}[Safe Active Learning]
\label{prob:3}
Given a state $x_i\in \stateset_0$, collect data that maximizes the reduction in uncertainty of $f$ while remaining in $\ProbControlSafeSet{\pi}$.
Periodically recompute $\ProbControlSafeSet{\pi}$ with the additional data, and continue until it is maximal.
\end{problem}

We begin by solving Problem~\ref{prob:1} with a novel control barrier formulation that explicitly accounts for learning the unknown function.
Gaussian process regression is performed to estimate the unknown function, and the resulting uncertainty estimates are used in the barrier function constraints. 
Then, the state and control hyperspace is coarsely partitioned and a recursive algorithm is employed to identify the safety-invariant set. 
Finally, Problem~\ref{prob:2} is solved with a greedy online exploration strategy that collects additional data, which is used to increase the safety-invariant set. 

% \subsection{Probability Measure}\label{prob:measure}
% \RM{Re-write following paragraph, from previous paper}
% \JS{I want to keep this separate from the problem above}
% The evolution of System~\eqref{Eqn:SystemEqn} can be characterized by the
% predictive posterior distribution ${\pdfx (\bar{x} \mid x)}$, which describes the probability density of $\pX_{k+1}$ when $\pX_k = x \in \reals^n$. 
% This distribution is induced by noise $\pV_k$ and hence is Gaussian with mean $\dyn$ and covariance $\cov$, i.e., ${
%     \pdfx (\bar{x} \mid x) = \N(\bar{x} \mid \dyn,\cov).}$
% For a subset of states $X \subseteq \reals^n$ and (initial) state $x\in \reals^n$, 
% we call 
% ${T(X \mid x) = \int_X \pdfx (\bar{x} \mid x) d \bar{x}}$ 
% the \emph{stochastic kernel} of System \eqref{Eqn:SystemEqn}. 
% From the definition of $T$ it follows that, for a given initial condition $\pX_0 = x_0 \in \reals^n$, $\pX_k$  is a Markov process with a well-defined probability measure $\Pr$ uniquely generated by the stochastic kernel $T$ \cite{bertsekas2004stochastic}. 
% For $X_0,X_k \subseteq \reals^n$, this probability measure is inductively defined as
% \begin{align*}
%     \Pr[\pX_0\in X_0] & =  \mathbf{1}_{X_0}(x_0) \\
%     \Pr[\pX_k\in X_k   \mid \pX_{k-1}=x]  & =  T^{}(X_k \mid x),
% \end{align*}
% where indicator function $\mathbf{1}_{X_0}(x_0) = 1$  if $x_0 \in X_0$, otherwise 0.
% The definition of $\Pr$ allows one to make probabilistic statements over the trajectories of System \eqref{Eqn:SystemEqn}.
% \RM{In this work, we are particularly interested obtaining control invariant sets that guarantee safety for System~\eqref{Eqn:SystemEqn}.}

% Safety set Definition
% \newcommand{\StateSet}{K}
% \newcommand{\SafeSet}{\StateSet_s}
% \newcommand{\pstar}{p^*}
% Let $\StateSet$ be a compact set. The set of safe states in $\StateSet$ is defined over horizon $N$ as
% \begin{align*}
% \SafeSet^N \coloneqq \{x_0\in\StateSet &\mid \Pr[\forall k\leq N, x_k\in\StateSet\mid x_{0}, u_{0:k-1}]\geq \pstar\}
% \end{align*}
% for some value of $\pstar$. 
% This definition relies on the existence of a control sequence $u_{0:k-1}\in U^k$ that results in $x_k\in\StateSet$.




% \begin{problem}[Control Invariant Set IMDP]
% Compute control invariant sets that satisfy some probability threshold using IMDPs
% \end{problem}

% We have a system, a data, verification of this system...

% \begin{problem}[Verification GPs]
%    \label{prob:1}
%    No confidence, probabilistic guarantees
% \end{problem}



==> bin/barrierSOS.tex <==
\RM{Theorem does not make sense, if probabilistic N-invariant sets is the aim, re-write }


\begin{theorem}[Control Invariant Set Barrier Certificate]
    \label{th:sosp_control_invariant}
    Consider SOS polynomial function $B(x)$, and
    safe set $ X_\safe = \set{  x \in \reals^{n} \mid h_{\safe}(x) \geq 0}$, 
    initial set $ X_{\initial} = \set{  x \in \reals^{n} \mid h_{\initial}(x) \geq 0}$, 
    unsafe set $X_{\unsafe} = \reals^n \setminus X_\safe = \set{  x \in \reals^{n} \mid h_{{\unsafe}}(x) \geq 0}$, and
    partition region $q= \set{  x \in \reals^{n} \mid h_{{q}}(x) \geq 0 }$ for all $q \in Q$.
    Let $\mathcal{L}_{\safe}(x)$, $\mathcal{L}_{\initial}(x)$ and $\mathcal{L}_{\unsafe}(x)$ be vectors of SOS polynomials with the same dimensions as $h_\safe$, $h_\initial$, and $h_\unsafe$, respectively. Likewise, let $\mathcal{L}_{q,x}(x)$  and $ \mathcal{L}_{a, u}(u)$
  be vectors of SOS polynomials with the same dimension as $h_q$ and $h_a$, respectively. 
   Then, a stochastic barrier certificate $B(x)$ for System~\eqref{eq:system} with time horizon $N \in \naturals_{\geq 0}$ can be obtained by solving the following SOS optimization problem for $\eta,\beta \in [0,1]:$
    \begin{subequations}
    \begin{align}
        &\min_{\beta,\eta} \quad \eta + \beta  N \qquad
         \text{subject to:} \nonumber \\
        & \hspace{5mm} B(x)\in \Lambda, \label{constraint1} \\
        &  \hspace{0.5 mm} - B(x) - \mathcal{L}^{T}_{\initial}(x)h_{\initial}(x) + \eta \in \Lambda, \label{constraint2}  \\
                & \RM{\eta \leq \eta_{\max}? } \\
        & \hspace{5mm} B(x) - \mathcal{L}^{T}_{\unsafe}(x)h_{\unsafe}(x) -1 \in \Lambda, \label{constraint3} \\
        % \begin{split}
                 & \hspace{.5mm} -E[B(f(\pX_{k}, \pU_{k}) + \pw) \mid x]  + B(x) + \beta_{q, a} -  \mathcal{L}^{T}_{q,x}(x)h_{q}(x)  \nonumber \\
                 & \hspace{7.5mm} - \mathcal{L}^{T}_{a,u}(u)h_{a}(u)\in \Lambda \hspace{10mm}   \label{constraint4}      
        \forall q \in Q, \forall a \in A
    \end{align}
    \end{subequations}
    This
    guarantees safety probability
    $P_\safe(X_\safe,X_0,N ) \geq 1 - (\eta + \beta N)$. 
\end{theorem}

\RM{Rewrite this proof for current implementation of CBF invariant set}

\RM{Theorem does not make sense, if control invariant barrier certificate is the aim, re-write }

==> bin/oldProbForm.tex <==
% \section{Problem Formulation \ml{OLD}}
% \label{sec:problem}

% \LL{I will add background on GP regression in here}
% \ml{should at least introduce the kernels and GPs very briefly before the assumption}
% \LL{Agree that is why I proposed to move the preliminaries before of Section 2}
% \ml{the GP alone makes a very short prelims section... it would be great to have both GPs and Barriers as prelims after problem formulation.}\LL{Issue with that is that for the probability measure we need to have introduced the posterior mean and variance. An alternative could be to introduce these directly in the problem formulation.}




% Given a set of data $D=\{(x_i,u_i,y_i),i\in\{1,...,|D|\}\}$ 
% generated by System~\eqref{eq:system}, for a given state and control input $(x,u)$ and a compact set $X \subseteq \mathbb{R}^n$, call $\sigma^2_D(x,u):=\kernel_D((x,u),(x,u))+R$. 
% We define the \emph{stochastic kernel} $T^D$ of  System~\eqref{eq:system} as 
% %\LL{I confirm, we need the preliminaries on GP regression before of this, because the kernel integrates the predictive posterior}
% \begin{align*}
% T^D(X \mid x,u ) := \int_{X} \mathcal{N}(z \mid \mu_D(x,u), \sigma^2_D(x,u)  )dz. 
% \end{align*}
% Then, for a given control strategy $\pi$, System~\eqref{eq:system} induces a probability measure $\Pr^{D,\pi}$, which is uniquely defined by $T^D$ and an initial condition such that~\cite{bertsekas2004stochastic}
% $$Pr^{D,\pi}(X \mid x)= T^D(X \mid x,\pi(x)) .$$
% %Similarly, given a strategy $\pi,$ we denote by $Pr^{\infty,\pi}$ the probability measure associated to system \eqref{Eqn:SystemEqn} when $f$ is known. That is, such that 
% %$$Pr^{\infty,\pi}(X \mid x)= \int_{X}\mathcal{N}(z\mid f(x,\pi(x)),R) .$$

% \subsection{Problem Statement}
% % with zero mean and covariance matrix $\cov \in \reals^{n \times n}$, $\N(\bar{x} \mid 0,\cov)$.
% %For a given state and control input $(x,u)$, the subsequent state $\pX'$ is distributed according to $\N(f(x,u),\cov)$.
% %Then, if $f$ were known, the probability of reaching $X\subset \reals^n$ is
% %\begin{equation}
% %\int_{X} \N(f(x,u),\cov) d x' \eqqcolon T(X \mid x,u)
% %\end{equation}
% %which is the \emph{stochastic kernel} of System~\ref{Eqn:SystemEqn}.
% %Using the stochastic kernel $T$ and a given $(x_0, u_0)$, $\mathbf{x}_k$ is a Markov process with a well-defined probability measure~\cite{bertsekas2004stochastic}.

% A general goal of this work is (active) safe learning of the dynamics.  The first step to such a problem is to compute the probability that System~\eqref{eq:system} remains within a compact safe set $X_\safe \subset \reals^n$ for a given time horizon. To this end, we introduce the notion of of \emph{probabilistic N-invariant set}, which is a subset of $X_\safe$ that System~\eqref{eq:system} does not exit with high probability for the next $N$ time steps if it starts from it.

% \begin{definition}[Probabilistic N-invariant set]
%     \label{def:invariant set}
%     Given a set of data $D$, a probability threshold $p^*,$ and a time horizon $N\in \mathbb{N}$,  we say that set $\ProbControlSafeSet{\pi} \subseteq X_{\safe}$ is the probabilistic N-invariant  for System~\eqref{eq:system} if there exists a strategy $\pi$ such that:
%     \begin{align}
%         \nonumber
%         \ProbControlSafeSet{\pi} =&\big\{ x\in X_{\safe}\, : \\ 
%         &\quad Pr^{D,\pi}[\forall k \leq N, \pX(k)\in \ProbControlSafeSet{\pi} \mid \pX(0)=x ] \geq p^* \big\}.
%         \nonumber
%     \end{align}
% \end{definition}
% The computation of the probabilistic N-invariant set  for System~\eqref{eq:system} is non-trivial. In fact, this requires not only to propagate the system dynamics over multiple time-steps, but also to account for the recursive nature of its definition. Consequently, the first problem we consider is that of computing the probabilistic N-invariant set.
% \begin{problem}[Probabilistic N-Invariant Set]
% \label{prob:1}
%     Given a set of data $D$, strategy $\pi,$ probability threshold $p^*,$ and time horizon $N\in \mathbb{N}$, find the probabilistic N-invariant set for System~\eqref{eq:system}.
% \end{problem}
% Given the available data, for each $\pi,$ $\ProbControlSafeSet{\pi}$ identifies the set of states from which not only System~\eqref{eq:system} remains safe for the next N time steps, but also with high probability remains only in states from which $N$-steps trajectories of the system are safe. This is employed in for active learning, where we continuously try to learn the system dynamics while remaining in states from which the system can be guaranteed to be safe, i.e., a safety controller exists.  In particular, in Problem \ref{prob:2} below, we seek a strategy that allows us to explore region of the state space with higher uncertainty, while remaining in a probabilistic N-invariant set. 





% In a safety-critical setting, the system must remain in the safe set, $X_\safe \subseteq \reals^n$.
% Computing the probability of remaining in $X_\safe$ from $x_0$ is straightforward using $T$ and a control sequence $\bar u_0^{N-1}=\{u_0,\dots,u_{N-1}\}$.
% Also, the system should be invariant with respect to safety, i.e. the terminal state $x_N$ should remain safe over a finite horizon.
% % Let the probability of System~\ref{Eqn:SystemEqn} remaining safe when initialized at $x_0$ in $N$ steps under control sequence $\bar u_0^{N-1}=\{u_0,\dots,u_{N-1}\}$ be
% % \JS{Think if there is a better way to handle control input sequences}
% % $$
% % p^N_{X_\safe}(x_0, \bar u_0^{N-1}) = \Pr[\forall k\leq N,x_k\in X_\safe \mid x_0,\bar u_0^{N-1}].
% % $$
% % With this definition, one can find all states and control inputs that satisfy the safety constraint $p^N_{X_\safe}(x_0, \bar u_0^{N-1})\geq p^*$.
% % However, this leaves an opportunity to reach a safe state where the safety probability is not satisfied.
% The set of states and control sequences that are invariant with respect to $\stateset_0\subseteq\stateset_\safe$ is
% \begin{align*}
% p^N_{\stateset_0}(x_0, \bar u_0^{N-1}) &= \Pr[\forall k\leq N,x_k\in X_0\mid x_0\in \stateset_0,\bar u_0^{N-1}].
% % &\leq \safethresh.
% \end{align*}
% This is the basis for the probabilistic \emph{safety-invariant set}, which is defined as
% \begin{align*}
% \ProbControlSafeSet \coloneqq \{
%     (x_0, \bar u_0^{N-1}) \in \stateset_0\times \controlset^{N-1} \colon
%     p^N_{\stateset_0}(x_0, \bar u_0^{N-1}) \geq \safethresh \}.
% \end{align*}

% Recall that the function $f$ is unknown \emph{a priori}, so we cannot reason about the transition kernel $T$ from the onset. 
% We assume the availability of a dataset consisting of one-step transitions, $\dataset=\{(x_i, u_i, x_{i+1})\}_{i=1}^\datasetsize$.
% We make the following assumption that will allow us to learn $f$ and quantify the learning uncertainty:
% \begin{assumption}
% % \label{ass:f}
% The unknown function $f$ is drawn from a Gaussian process prior model $\mathcal{GP}(\mu_0,\kernel_0)$.
% \end{assumption}
% Details about this assumption can be found in Section~\ref{sec:GPs}.
% \JS{This assumption can be made even more general, such as:}
% \begin{assumption}\label{ass:f2}
% Let $X$ be a compact set. 
% The unknown function $f$ can be estimated from the dataset $\dataset$ such that the error between the estimate $\hat f$ and $f$ is probabilistically bounded as
% $$
% \Pr[\forall x\in X, \|f - \hat f\| < \epsilon]\geq 1-\delta.
% $$
% \end{assumption}
% \textcolor{blue}{This assumption admits any suitable regression method to estimate $\hat f$. 
% In the setting of GP regression, the standard case, uniform error bounds (Lederer 2020), and the agnostic case (RKHS, Chowdhury 2017) are all applicable.
% This paper focuses on the standard case without loss of generality.
% }



==> sections/Appendices/1_GP_bounding.tex <==
\section{Misc}

Probably not useful

\subsection{GP Bounding Adjustment}
\JS{This is more of an implementation detail.}
In Section .. , the proposed GP formulation takes the form 
$$
   x_{k+1}  = \Gm + \Gv.
$$
To facilitate better regression with GPs, we learn the change the current point $x_k$, or
$$
x_{k+1} = x_k + \Gm + \Gv.
$$
which is equivalent to setting a prior mean function that relies on $x$, i.e. $m_0(x) = x$. 
Therefore, given $x_k$ and bounds $[\lGm, \uGm]$, 
$$
x_{k+1} \in [x_k + \lGm, x_k + \uGm].
$$
Likewise, given an interval of possible inputs, $[x^L_k, x^U_k]$, the range of possible outputs is $[x^L_{k+1}, x^U_{k+1}]$ where \JS{incorrect notation below for mean bounds over interval}
$$
x^L_{k+1} = x^L_k + \lGm,~~x^U_{k+1} = x^U_k + \uGm
$$

\subsection{Polynomial Kernel}
The polynomial kernel is

\begin{align}
\kernel(x_1,x_2) &= \var(x_1'x_2 + c)^d
\end{align}

So the posterior mean is (zero prior)
$$
\mean(x) = \sum_{j=1}^m\var\alpha_j(x'x_j+c)^d
$$
and the posterior variance (conditioned on the dataset $D$) is 
$$
\std_\dataset^2(x) = \var(x'x+c)^d-\sum_{i=1}^\datasetsize \var(x'x_i+c)^d\sum_{j=1}^\datasetsize K^{-1}_{i,j}\var(x'x_j+c)^d
$$
where $\datasetsize=|\dataset|$ is the size of the training dataset.
In addition, the total variance is this posterior variance plus the noise variance:
$$
\std_{total}^2(x) = \var(x) + R
$$

\subsection{Exponential Kernel}

Bounds on GP:

$$\tilde{A}
+
\tilde{C}
+
\tilde{B} x^{T} \theta I x
-
\tilde{D}x
\geq \mu(x)
\geq 
A
+
C
+
B x^{T} \theta I x
- Dx
$$

\subsection{Random Tools}
https://en.wikipedia.org/wiki/Pad%C3%A9_approximant

Upper bound based on :

https://stackoverflow.com/questions/42732225/fast-integer-sqrt-upper-bound-approximation

==> sections/Appendices/2_BarrierSOS.tex <==
\section{Sum-of-Squares Barrier}

Using piecewise barrier now

The synthesis of a stochastic barrier certificate can be formulated as a nonlinear optimization problem, which can be solved efficiently using convex optimization. We define an SOS polynomial as

\begin{definition}[SOS Polynomial]
    \label{def:sosp1}
    A multivariate polynomial $\lambda(x)$ is  a Sum-Of-Squares (SOS) for $x \in \mathbb{R}^{n}$ if there exists some polynomials $\lambda_{i}$, $i = 1, \ldots, r$, for some ${r \in \naturals}$, such that
    $\lambda(x) = \sum_{i=1}^{r} \lambda_{i}^{2}(x) \geq 0.$
    % If $\lambda(x)$ is an SOS, then $\lambda(x) \geq 0$ for all $x \in \mathbb{R}^{n}$. 
    The set of all SOS polynomials is denoted by $\Lambda$.
\end{definition}

Consider a basic closed semi-algebraic set $X =\set{x \in \reals^n \mid h_i(x) \geq 0  \;\; \forall i \in \set{1, \ldots, l}}$, which is defined as the intersection of $l$ polynomial ($h_i(x)$) inequalities. 
\begin{proposition}[Putinar’s Certificate, \cite{Stengle1974}]
    \label{prop:sosp1}
    Polynomial $\gamma(x)$ is non-negative on $X$ if,   for some $ \lambda_{0}(x), \lambda_{i}(x) \in \Lambda$,
    % \begin{equation*}
        $\gamma (x) = \lambda_0(x) + \sum_{i=1}^{l} \lambda_{i}(x) h_{i}(x).$
    % \end{equation*}
\end{proposition}

Using these properties, Theorem \ref{th:sosp_gpbarrier} shows how the Probabilistic N-Invariant sets can be obtained for a GP model using a barrier approach. In particular, the theorem shows how to formulate Conditions -- as SOS constraints. 

\RM{Combine theorem 1 and 2 into 1...}


% \begin{proof}
% It suffices to show that if $B$ satisfies Constraints \eqref{constraint1}-\eqref{constraint4}, then Conditions \eqref{Eq:Cond3}-\eqref{Eq:Cond5} are satisfied. 
% As Constraint \eqref{constraint1} guarantees that $B$ is a SOS polynomial, hence non-negative by definition, Condition \eqref{Eq:Cond3} holds. 
% By Corollary \ref{cor:sosp1} it holds that if Constraints \eqref{constraint2}-\eqref{constraint3} hold, then $B$ is respectively smaller that $\eta$ in $X_0$ and greater than $1$ in $X_u$. What is left to show is that Constraint \eqref{constraint4} guarantees the satisfaction of Condition \eqref{Eq:Cond5}. This can be done as follows. 
% For every region $q \in Q$,
% the expectation term in Condition \eqref{Eq:Cond5} can be expressed as $E[B(y + v) \mid x]$, where $y$ is bounded by under-approximation $\low{f}_q(x)$ and over-approximation $\up{f}_q(x)$ of $\NN(x)$ in System \eqref{Eqn:SystemEqn}  for all $x \in q$.  Then by Corollary \ref{cor:sosp1}, Constraint \eqref{constraint4} is obtained for each $q$.  Note that $B(x)$ is a polynomial, so if $E[B(y + v) \mid x]$ is also a polynomial, the condition is a valid SOS constraint.  Given that $y + v$ is linear, $E[B(y + v) \mid x]$ is a sum of monomials in terms of $y$ and expectation moments $\mathbb{E}[v^{d}]$, where $d \geq 0$. Since, random variable $v$ has a normal distribution, $\mathbb{E}[v^{d}]$ is  constant.  Therefore, $E[B(y + v) \mid x]$ is a polynomial only in terms of (components of) $y$. 
% \end{proof}

\RM{Remove SOS formulation}

\begin{theorem}[Probabilistic N-Invariant Sets]
    \label{th:sosp_gpbarrier}
    Consider SOS polynomial function $B(x)$, and
    % sets
    % \begin{itemize}
    %     \item safe set $ X_\safe = \set{  x \in \reals^{n} : h_{\safe}(x) \geq 0}$, 
    %     \item initial set $ X_{\initial} = \set{  x \in \reals^{n} : h_{\initial}(x) \geq 0}$, 
    %     \item unsafe set $X_{\unsafe} = \reals^n \setminus X_\safe = \set{  x \in \reals^{n} : h_{{\unsafe}}(x) \geq 0}$, and
    %     \item partition region $X_q= \set{  x \in \reals^{n} : h_{{q}}(x) \geq 0 }$ for all $q \in Q$.
    % \end{itemize}
    safe set $ X_\safe = \set{  x \in \reals^{n} \mid h_{\safe}(x) \geq 0}$, 
    initial set $ X_{\initial} = \set{  x \in \reals^{n} \mid h_{\initial}(x) \geq 0}$, 
    unsafe set $X_{\unsafe} = \reals^n \setminus X_\safe = \set{  x \in \reals^{n} \mid h_{{\unsafe}}(x) \geq 0}$, and
    partition region $q= \set{  x \in \reals^{n} \mid h_{{q}}(x) \geq 0 }$ for all $q \in Q$.
    Let $\mathcal{L}_{\safe}(x)$, $\mathcal{L}_{\initial}(x)$ and $\mathcal{L}_{\unsafe}(x)$ be vectors of SOS polynomials with the same dimensions as $h_\safe$, $h_\initial$, and $h_\unsafe$, respectively. Likewise, let $\mathcal{L}_{q,x}(x)$  and $ \mathcal{L}_{q, m}(x)$ be vectors of SOS polynomials with the same dimension as $h_q$ and $\Gm$, respectively. Finally, let $\mathcal{L}_{q}(\std)$ be a $n$-dimensional vector of polynomials.
   Then, a stochastic barrier certificate $B(x)$ for System~\eqref{eq:system} with time horizon $N \in \naturals_{\geq 0}$ can be obtained by solving the following SOS optimization problem for $\eta,\beta \in [0,1]:$
    \begin{subequations}
    \begin{align}
        % \label{eq:OptimProb}
        &\min_{\beta,\eta} \quad \eta + \beta  N \qquad
         \text{subject to:} \nonumber \\
        & \hspace{0.5mm} B(x)\in \Lambda, \label{constraintGP1} \\
        \hspace{0.5mm} - &  B(x) - \mathcal{L}^{T}_{\initial}(x)h_{\initial}(x) + \eta \in \Lambda, \label{constraintGP2}  \\
        & \hspace{0.5mm} B(x) - \mathcal{L}^{T}_{\unsafe}(x)h_{\unsafe}(x) -1 \in \Lambda, \label{constraintGP3} \\
        % \begin{split}
                 & \hspace{0.5mm} -E[B( y + {v}) \mid x]  + B(x) /\alpha + \beta -  \mathcal{L}^{T}_{q,x}(x)h_{q}(x) - \nonumber \\
                 & \hspace{7.5mm} \mathcal{L}^{T}_{q, m}(x)
                 \left (
                 (\lGm - m)\odot(m - \uGm)
                 \right ) - 
                 \\
                & \hspace{7.5mm}
                 \mathcal{L}^{T}_{q}(\std)
                  \left (
                 (\up{\std}_q - \std)\odot(\std - \low{\std}_q)
                 \right ) 
                 \in \Lambda \hspace{10mm}   \label{constraintGP4}      
        % \end{split}
        \forall q \in Q
    \end{align}
    \end{subequations}
    where $\odot$ denotes the element-wise Schur product. This
    guarantees safety probability
    $P_\safe(X_\safe,X_0,N ) \geq 1 - (\eta + \beta N)$. 
\end{theorem}


==> sections/Appendices/3_ActiveLearning.tex <==
\section{Active Learning}

Active learning is an intelligent procedure to collect additional data to satisfy an objective. 
Our objective is to increase the size of the control invariant set while remaining safe. 

Our active learning procedure uses a greedy action-selection criterion on the discrete states $Q$, and the continuous space $X$. 

This criterion is the maximum variance according to the posterior GP given the current dataset $D_k$ where $k$ denotes the current step in the online setting. 
Recall for a given point $(x,u)$, the posterior variance is $\var(x,u)$ and for discrete state $q=\{[x_L, x_U], [u_L,u_U]\}$ the variance for all points therein is upper-bounded by $\up\var(q)$.

\subsection{Discrete Control Selection}
Given the current state $x_k$, the most valuable control interval according to $\up\var(q)$. 

The motivation behind choosing the interval first is that 1) the interval has already been deemed safe, so we know the system will remain safe with high probability for any action selected from the interval, and 2) choosing the interval where there is the highest uncertainty $\up\var(q)$ means the most information stands be be collected.


\subsection{Continuous Control Selection}
After the best control interval is chosen, it remains to find the value of the continuous control $u_k$ in the interval that maximizes $\var(x_k,u_k)$. 
For the squared-exponential kernel, this can be done by employing bounds. 
Otherwise, a suboptimal choice of $u_k$ can be found via sampling the GP posterior.
This can be done cheap and fast, online. 

\subsection{Barrier Updates}
\JS{Current setup with barriers only lets us reason about the control. GPs can be used to reason about states we want to reach from $x_k$}
Once a control input is selected and executed, the resulting datapoint $(x_k, u_k, x_{k+1})$ can be used to update the GP regression, and in turn update the CBFs and control invariant set. 

As we have already identified some control invariant sets, we can focus on finding improvements in other non-safe sets. 
Let $Q^?$ be the set of possibly control invariant sets. 
Since we draw the control from interval $[u]$, we can try updating all states with $[u]\in q$. 

There are two options for updating the barrier:
\begin{itemize}
    \item Re-evaluate the barrier polynomial to get new values of $\beta$, 
    \item Recompute the barrier entirely
\end{itemize}
We provide a brief comparison of these two approaches in the case studies.

\subsubsection{No Safe Intervals}
What happens if, after executing a safe action $u_k$, the system enters a region $q$ that contains no control intervals that are safe with at least probability $p^*$? 
Can we reason \emph{a prior} about states where we can return %to $\ControlSafeSet$ in one step if we end up in them? 
Or are these actually not a concern?



==> sections/Appendices/4_Derivations.tex <==

\subsection{PWCB}

\RM{Still think about this...}

\begin{theorem}[Piecewise Barrier with Partitioned Control]
Assume a piecewise function $B_i(x)$ over state partition $X_s = \cup_{i=1}^I X_i$, $x \in X_i $, 
control partition $U = \cup_{k=1}^K U_k$, $u \in U_k$, 
and stochastic process $\px' = f(x, u, v) $.
%, and time horizon $H\in \mathbb{N}$.
%Consider a piece-wise barrier $B_i(x)$ over the $i^{th}$ partition in set $X_s = \{X_1, \ldots, X_k \}$. 
% Then, $B(x) = \cup_{i=1}^K B_i(x)$ 
% is a piecewise stochastic barrier function if $\phantom{.} \forall i,j = \{1,\ldots, K\}$ $\exists \beta_j: X_j \to \mathbb{R}$ and $\exists \eta\geq 0$ such that the following conditions hold
\begin{subequations} 
    \begin{align}
        & B_{j}(x)\geq 0   &&  \hspace{-15mm} \forall j
        %\label{Eq:Cond3}
        \\ 
        & B_{j}(x)\leq \eta  && \hspace{-15mm} \forall j : X_j \cap X_0, \neq \emptyset
        \\
        & \indicator{B(x)} = 1  && \hspace{-15mm}\forall j : X_j \cap X_u, \neq \emptyset\\
        & \sum_{i = 1}^K \expect[B_i(\px') \mid \px' \in X_i] \cdot p(\px' \in X_i) && \nonumber \\
        & \quad + \indicator{X_u}(\px') \cdot p(\px' \in X_\unsafe)   \leq  B_{j}(x) + \beta_{j} && \forall x \in X_j  
   %\label{Eq:Cond5}
    \end{align}
\end{subequations}
Minimization over the objective $\eta + N\cdot \max \beta_j$ guarantees safety probability $P_\safe(X_\safe,X_0, N) \geq 1 - (\eta + N\cdot \max \beta_j)$. 
\end{theorem}
